Towards Robustness to Label Noise in Text Classification via Noise Modeling

Large datasets in NLP suffer from noisy labels, due to erroneous automatic and human annotation procedures. We study the problem of text classification with label noise, and aim to capture this noise through an auxiliary noise model over the classifier. We first assign a probability score to each training sample of having a noisy label, through a beta mixture model fitted on the losses at an early epoch of training. Then, we use this score to selectively guide the learning of the noise model and classifier. Our empirical evaluation on two text classification tasks shows that our approach can improve over the baseline accuracy, and prevent over-fitting to the noise.

==> inp_tables.tex <==
\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cclccclccc}
\toprule
                                                                               &          &  & \multicolumn{3}{c}{\textbf{`How'/`What' based}}       &  & \multicolumn{3}{c}{\textbf{Question Length based}}     \\  \cmidrule(lr){4-6} \cmidrule(l){8-10} 
Model                                                                          & Noise \% &  & Base & $\mathcal{H}$ & $\mathcal{S}$ &  & Base & $\mathcal{H}$ & $\mathcal{S}$ \\ \midrule
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}word\\ LSTM\end{tabular}}}  & 10       &  & 89.2     & \textbf{91.8}        & 91.8                 &  & 91.4     & 91.6                 & \textbf{92.0}        \\
                                                                               & 20       &  & 84.4     & 87.4                 & \textbf{90.6}        &  & 87.0     & 90.2                 & \textbf{90.6}        \\
                                                                               & 30       &  & 77.8     & \textbf{84.2}        & 83.8                 &  & 82.2     & \textbf{87.4}        & 85.4                 \\
                                                                               & 40       &  & 76.0     & 79.0                 & \textbf{79.2}        &  & 82.4     & \textbf{87.4}        & 84.0                 \\
                                                                               & 50       &  & 71.8     & 67.8                 & \textbf{75.6}        &  & 74.2     & \textbf{79.0}        & 75.0                 \\ \midrule
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}word\\ CNN\end{tabular}}}  & 10       &  & 90.4     & 90.0                 & \textbf{91.2}        &  & 91.0     & 90.6                 & \textbf{92.8}        \\
                                                                               & 20       &  & 83.8     & 86.6                 & \textbf{86.8}        &  & 88.0     & 89.6                 & \textbf{91.0}        \\
                                                                               & 30       &  & 82.4     & \textbf{84.4}        & 84.2                 &  & 85.2     & \textbf{87.2}        & 86.8                 \\
                                                                               & 40       &  & 78.8     & 80.6                 & \textbf{81.8}        &  & 82.0     & 82.6                 & \textbf{86.0}        \\
                                                                               & 50       &  & 52.0     & \textbf{74.0}        & 65.2                 &  & 73.6     & \textbf{77.0}        & 75.4                 \\ \bottomrule
\end{tabular}%
}
    \captionof{table}{Input-conditional noise on TREC.}
    \label{tab:inp_trec_results}
\end{table}

\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
               &  & \multicolumn{3}{c}{\textbf{word LSTM}}                       &  & \multicolumn{3}{c}{\textbf{word CNN}}                                                                                    \\ \cline{3-5} \cline{7-9} 
Noise Type (\%)     &  & Base & $\mathcal{H}$ & $\mathcal{S}$ &  & \multicolumn{1}{c}{Base} & \multicolumn{1}{c}{$\mathcal{H}$} & \multicolumn{1}{c}{$\mathcal{S}$} \\ \midrule
AP (7.8 \%)         &  & 82.8     & 82.7                    & \textbf{82.8}           &  & \textbf{83.1}                & 82.4                                        & 82.5                                        \\
Reuters (10.8\%)    &  & 85.6     & \textbf{85.7}           & 85.5                    &  & 85.7                         & \textbf{86.2}                               & 86.1                                        \\
AP+Reuters (18.6\%) &  & 75.7     & \textbf{76.6}           & 76.0                    &  & \textbf{76.6}                & 76.1                                        & 76.4                                        \\ \bottomrule
\end{tabular}%
}
\captionof{table}{
Results from input-conditional noise on AG-News. $\mathcal{H/S}$ denotes $\mathcal{L_{DN{-}H/S}}$.
}
\label{tab:inp_ag_results}
\end{table}


==> model_figure.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp9465494322222059] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (120.5,100.33) -- (180.5,100.33) -- (180.5,170.33) -- (120.5,170.33) -- cycle ;
%Straight Lines [id:da283535857086862] 
\draw    (180,164.33) -- (229,164.33) ;
\draw [shift={(231,164.33)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp7378282575642985] 
\draw  [fill={rgb, 255:red, 246; green, 146; blue, 146 }  ,fill opacity=1 ] (231,100.33) -- (262.5,100.33) -- (262.5,170.33) -- (231,170.33) -- cycle ;
%Straight Lines [id:da25833269503700595] 
\draw    (207.5,137.33) -- (207.5,98.33) ;
\draw [shift={(207.5,96.33)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6633319068062542] 
\draw    (179.5,137.33) -- (207.5,137.33) ;
%Straight Lines [id:da9855374208388115] 
\draw    (278.5,138.33) -- (278.5,98.33) ;
\draw [shift={(278.5,96.33)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7789034335768101] 
\draw    (263.5,138.33) -- (278.5,138.33) ;
%Straight Lines [id:da3817991440147501] 
\draw    (91.5,134.33) -- (118.5,134.33) ;
\draw [shift={(120.5,134.33)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da694942842812827] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (205.5,67.33) -- (205.5,60.33) ;
%Straight Lines [id:da8197975165757654] 
\draw [color={rgb, 255:red, 91; green, 157; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=1 ]   (153.5,81.33) -- (196.5,81.33) ;
%Straight Lines [id:da9389945940788857] 
\draw [color={rgb, 255:red, 91; green, 157; blue, 19 }  ,draw opacity=1 ]   (153.5,81.33) -- (153.5,48.33) ;
\draw [shift={(153.5,46.33)}, rotate = 450] [color={rgb, 255:red, 91; green, 157; blue, 19 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da13909626106842943] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (205.5,60.33) -- (278.5,60.33) ;
%Straight Lines [id:da9256583745840932] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (278.5,67.33) -- (278.5,60.33) ;
%Straight Lines [id:da30940705553991377] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (239.5,60.33) -- (239.5,47.33) ;
\draw [shift={(239.5,45.33)}, rotate = 450] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (202,68.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 90; green, 160; blue, 13 }  ,opacity=1 ]  {$\hat{y}_{c}$};
% Text Node
\draw (271,67.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\hat{y}_{n}$};
% Text Node
\draw (75,124.4) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (186,149.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$R_{M}( x)$};
% Text Node
\draw (142,126.4) node [anchor=north west][inner sep=0.75pt]    {$M$};
% Text Node
\draw (234,123.4) node [anchor=north west][inner sep=0.75pt]    {$N_{M}$};
% Text Node
\draw (201,31.4) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\text{Train with} \ L_{DN}$};
% Text Node
\draw (129,33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 94; green, 167; blue, 15 }  ,opacity=1 ] [align=left] {Inference};


\end{tikzpicture}

